Gate-Shift-Fuse for Video Action Recognition

Convolutional Neural Networks are the de facto models for image recognition. However 3D CNNs, the straight forward extension of 2D CNNs for video recognition, have not achieved the same success on standard action recognition benchmarks. One of the main reasons for this reduced performance of 3D CNNs is the increased computational complexity requiring large scale annotated datasets to train them in scale. 3D kernel factorization approaches have been proposed to reduce the complexity of 3D CNNs. Existing kernel factorization approaches follow hand-designed and hard-wired techniques. In this paper we propose Gate-Shift-Fuse (GSF), a novel spatio-temporal feature extraction module which controls interactions in spatio-temporal decomposition and learns to adaptively route features through time and combine them in a data dependent manner. GSF leverages grouped spatial gating to decompose input tensor and channel weighting to fuse the decomposed tensors. GSF can be inserted into existing 2D CNNs to convert them into an efficient and high performing spatio-temporal feature extractor, with negligible parameter and compute overhead. We perform an extensive analysis of GSF using two popular 2D CNN families and achieve state-of-the-art or competitive performance on five standard action recognition benchmarks.

==> sub/5_sup.tex <==
\section*{Impact of Learnable Fusion}

Fig.~\ref{fig:gsmvgsf} compares the class categories that are improved by adding the proposed fusion mechanism to GSM. We can see that the fusion mechanism improves the model’s capability to recognize categories that have a similar temporal structure but slightly different visual (static) information such as \texttt{Uncovering something} vs \texttt{Removing something, revealing something behind}, \texttt{Putting something behind something} vs \texttt{Pretending to put something something behind something}, \etc. We show the saliency tube visualization of two samples, where GSM failed and GSF succeeded in correctly recognizing the class category, in Fig.~\ref{fig:visualization_gsmf}. In Fig.~\ref{fig:uncovering}, GSM focuses more on the state of the object(s) before and after the action is carried out while GSF makes the prediction by focusing on the frames just before the action, during the action and just after the action. Similarly, in Fig.~\ref{fig:putting_behind}, GSF starts focusing on the frame when the object is introduced to the scene and continues to focus on the object even after the hand is removed while GSM made the decision based on the frames after the hand starts to be visible in the scene. This shows that the fusion mechanism enables an additional flexibility to the model in selecting how much of the dynamic (from shifted features) and static (from residual features) information to be encoded. This allows the model to better represent the state changes occurring to the object(s) in the scene correctly, leading to an improved recognition performance.

\begin{figure*}[h]
	\centering
	\includegraphics[scale=0.5]{supplemental/figures/gsm_v_gsf_cropped.png}
	\caption{Action classes with the highest improvement by applying the weighted fusion to GSM. X-axis shows the the number of corrected samples for each class. Y-axis labels are in the format true label (GSF)/predicted label (GSM).}
	\label{fig:gsmvgsf}
\end{figure*}


\begin{figure*}[t]
	\centering
	\begin{subfigure}[b]{0.005\textwidth} 
		\raisebox{0.8cm}{\rotatebox[origin=c]{90}{GSM}}
	\end{subfigure} \hskip -3mm
	\begin{subfigure}[b]{0.95\textwidth}
		\centering
		\includegraphics[scale=0.25]{./supplemental/figures/uncovering_something/gsm/000.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/uncovering_something/gsm/001.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/uncovering_something/gsm/002.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/uncovering_something/gsm/003.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/uncovering_something/gsm/004.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/uncovering_something/gsm/005.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/uncovering_something/gsm/006.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/uncovering_something/gsm/007.png}
	\end{subfigure} \\[1mm]
	\begin{subfigure}[b]{0.005\textwidth} 
		\raisebox{1.4cm}{\rotatebox[origin=c]{90}{GSF}}
	\end{subfigure} \hskip -3mm
	\begin{subfigure}[b]{0.95\textwidth}
		\centering
		\includegraphics[scale=0.25]{./supplemental/figures/uncovering_something/gsf/000.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/uncovering_something/gsf/001.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/uncovering_something/gsf/002.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/uncovering_something/gsf/003.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/uncovering_something/gsf/004.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/uncovering_something/gsf/005.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/uncovering_something/gsf/006.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/uncovering_something/gsf/007.png} 
		\caption{\texttt{uncovering something}}
		\label{fig:uncovering}
	\end{subfigure} \\ \vskip 3mm
	\begin{subfigure}[b]{0.005\textwidth} 
		\raisebox{0.8cm}{\rotatebox[origin=c]{90}{GSM}}
	\end{subfigure} \hskip -3mm
	\begin{subfigure}[b]{0.95\textwidth}
		\centering
		\includegraphics[scale=0.25]{./supplemental/figures/putting_something_behind_something/gsm/000.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/putting_something_behind_something/gsm/001.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/putting_something_behind_something/gsm/002.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/putting_something_behind_something/gsm/003.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/putting_something_behind_something/gsm/004.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/putting_something_behind_something/gsm/005.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/putting_something_behind_something/gsm/006.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/putting_something_behind_something/gsm/007.png}
	\end{subfigure} \\[1mm]
	\begin{subfigure}[b]{0.005\textwidth} 
		\raisebox{1.4cm}{\rotatebox[origin=c]{90}{GSF}}
	\end{subfigure} \hskip -3mm
	\begin{subfigure}[b]{0.95\textwidth}
		\centering
		\includegraphics[scale=0.25]{./supplemental/figures/putting_something_behind_something/gsf/000.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/putting_something_behind_something/gsf/001.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/putting_something_behind_something/gsf/002.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/putting_something_behind_something/gsf/003.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/putting_something_behind_something/gsf/004.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/putting_something_behind_something/gsf/005.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/putting_something_behind_something/gsf/006.png}\hskip 1mm
		\includegraphics[scale=0.25]{./supplemental/figures/putting_something_behind_something/gsf/007.png} 
		\caption{\texttt{putting something behind something}}
		\label{fig:putting_behind}
	\end{subfigure}
	\caption{Saliency tubes generated by GSM (top) and GSF (bottom) on sample videos taken from the validation set of Something Something-V1 dataset.}
	\label{fig:visualization_gsmf}
\end{figure*}

\section*{Runtime Analysis}
In this section, we report additional runtime analaysis performed on GSF. Firstly, we compute the latencies incurred by various operations that are performed in GSF. The results of this analysis is reported in Tab.~\ref{tab:gsf_breakdown} (please see the PyTorch style pseudocode provided in Fig.~\ref{code:gsf} for details of each operation). We report the average of the latencies incurred by all GSF layers in the ResNet-50 backbone. From the table one can see that the 3D convolution operation used for computing the gating values is the main source of delay in GSF. 

To further verify that the 3D convolution, in GSF, that generates a single channel gating output performs better than the standard full 3D convolution (used in 3D CNNs) both in terms of accuracy and latency, we perform an additional analysis by computing the latency of a single GSF video recognition block. We define a GSF video recognition block as defined in Fig.~5 in the main paper (GSF plugged in after the third 2D Conv of ResNet Bottleneck block). Tab.~\ref{tab:block_comparison} reports the latency incurred by various video recognition blocks. We apply the same input of dimension $1\times8\times256\times56\times56$ as input to all blocks. It should be noted that all models are run at half precision except for RubiksNet since its public implementation\footnote{\url{https://github.com/StanfordVL/RubiksNet}} do not support half precision. From the table, we can see that GSF performs better than Conv3D model both in terms of accuracy and latency. On the other hand, compared to TSM and RubiksBlock, GSF is slighly slower but results in an accuracy improvement of $+4.5\%$ and $+3.7\%$, respectively.

\begin{table}[t]
	\centering
	\begin{tabular}{|c|c|}
		\hline 
		Step & Time \\ \hline
		Pre-processing &  $454\mu s$ \\
		Gate computing &  $2.675ms$ \\
		Gating &  $366\mu s$ \\
		Shifting &  $188\mu s$ \\
		Fusion weight computing &  $618\mu s$ \\
		Fusion &  $0.0\mu s$ \\
		Post-processing &  $335\mu s$ \\ \hline
		\hline 
		Total & $4.636ms$  \\ \hline
	\end{tabular}
	\caption{Detailed latency of each operation performed in GSF}
	\label{tab:gsf_breakdown}
\end{table}
\begin{table}[t]
	\centering
	\begin{tabular}{|c|c|c|}
		\hline 
		Block & Time (ms) & Accuracy (\%)  \\ \hline
		Conv3D &  $2.673$ & 45.8\\
		% R(2+1)D &  $3.656ms$ & 47.3\\
		TSM &  $1.285$ & 45.6\\
		RubiksBlock$^*$ &  $1.252$ & 46.4\\
		\hline
		\hline 
		GSF & $1.655ms$ & 50.17\\ \hline
	\end{tabular}
	\caption{Latency of various video recognition blocks. The input to the block is a fixed tensor with a batch size of 1, channels 256, temporal dimension 8 and spatial dimensions 56$\times$56. We also report the accuracy on the validation set of Something-V1 dataset. \revnewvt{}{$^*$: All blocks except RubiksBlock are run with half precision.}}
	\label{tab:block_comparison}
\end{table}



\begin{figure*}
	\begin{minted}{python}
	# Pre-processing
	x = x_full[:, :self.fPlane, :, :]
	batchSize = x.size(0) // self.num_segments
	shape = x.size(1), x.size(2), x.size(3)
	x = x.view(batchSize, self.num_segments, *shape).permute(0, 2, 1, 3, 4)
	x_bn = self.bn(x)
	x_bn_relu = self.relu(x_bn)
	# Gate computing
	gate = self.tanh(self.conv3D(x_bn_relu))
	# Gating
	gate = gate.reshape(
	batchSize, 2, 1, self.num_segments, shape[1], shape[2]
	).expand(-1, -1, shape[0]//2, -1, -1, -1
	).reshape(
	batchSize, shape[0], self.num_segments, shape[1], shape[2])
	y = torch.mul(gate, x)
	r = torch.sub(x, y)
	# Shifting
	out_shifted = torch.zeros_like(y)
	out_shifted[:, :y.size(1)//2, :-1] = y[:, :y.size(1)//2, 1:]  # shift left
	out_shifted[:, y.size(1)//2:, 1:] = y[:, y.size(1)//2:, :-1]  # shift right
	y = out_shifted
	# Fusion weight computing
	y_group1, y_group2 = y.split([self.fPlane//2, self.fPlane//2], dim=1)
	r_group1, r_group2 = r.split([self.fPlane//2, self.fPlane//2], dim=1)
	y_1 = torch.nn.functional.adaptive_avg_pool2d(y, (1)).view(batchSize, shape[0],
	self.num_segments)
	r_1 = torch.nn.functional.adaptive_avg_pool2d(r, (1)).view(batchSize, shape[0], 
	self.num_segments)
	y_r = torch.stack([y_1, r_1], dim=1)
	y_r_1, y_r_2 = y_r.split([self.fPlane//2, self.fPlane//2], dim=2)
	y_1_weights = torch.sigmoid(y_r_1).view(batchSize, channels, num_segments, 1, 1)
	r_1_weights = 1 - y_1_weights
	y_2_weights = torch.sigmoid(y_2_1).view(batchSize, channels, num_segments, 1, 1)
	r_2_weights = 1 - y_2_weights
	# Fusion
	y_group1 = y_group1*y_1_weights + r_group1*r_1_weights
	y_group2 = y_group2*y_2_weights + r_group2*r_2_weights
	# Post-processing
	y_group1 = y_group1.view(batchSize, 2, self.fPlane // 4, self.num_segments, *shape[1:]
	).permute(0, 2, 1, 3, 4, 5)
	y_group2 = y_group2.view(batchSize, 2, self.fPlane // 4, self.num_segments, *shape[1:]
	).permute(0, 2, 1, 3, 4, 5)
	
	x_full[:, :self.fPlane, :, :] = torch.cat(
	(y_group1.reshape(
	batchSize, self.fPlane//2, self.num_segments,
	*shape[1:]
	),
	y_group2.reshape(
	batchSize, self.fPlane//2, self.num_segments, 
	*shape[1:]
	)
	), dim=1).permute(0, 2, 1, 3, 4).reshape(
	batchSize * self.num_segments, *shape
	)
	\end{minted}
	\caption{PyTorch style pseudo code of GSF layer.}
	\label{code:gsf}
\end{figure*}

==> sub/changes.tex <==
\color{red}
\section{Changes}
1. Learned Fusion

\noindent 2. Backbone CNNs. Extend GSM to ResNet family of CNNs. This requires additional ablation studies, as reported in the rebuttal.

\noindent 3. New datasets. We could extend the current version by including the following datasets:
\begin{itemize}
    \item Something-V2: Same as Something-V1, with more samples, less label noise and higher resolution images.
    \item Kinetics: This could be tricky as it do not require strong spatio-temporal reasoning. However, can be used to pre-train the model for evaluation in other datasets. Something datasets could also benefit from the pre-training.
    \item EPIC-KITCHENS 100
\end{itemize}

\noindent 4. New tasks: Action localization, detection. 

If we manage to train with one of the large scale datasets, we may use the pre-trained network for other tasks such as video captioning, video question answering, action detection, \etc, by replacing 3D CNNs with TSN+GSM on available codes.

\color{black}
